A Primer on Causal and Statistical Dataset Biases for Fair and Robust Image Analysis

Machine learning methods often fail when deployed in the real world. Worse still, they fail in high-stakes situations and across socially sensitive lines. These issues have a chilling effect on the adoption of machine learning methods in settings such as medical diagnosis, where they are arguably best-placed to provide benefits if safely deployed. In this primer, we introduce the causal and statistical structures which induce failure in machine learning methods for image analysis. We highlight two previously overlooked problems, which we call the \textit{no fair lunch} problem and the \textit{subgroup separability} problem. We elucidate why today's fair representation learning methods fail to adequately solve them and propose potential paths forward for the field.

==> bibstyle.tex <==
% An actually decent referencing style. C. Jones 2025.
\PassOptionsToPackage{
    style=authoryear, % Harvard/APA ish
    backend=bibtex, 
    natbib=true, % use \citep, \citet
    backref=true, % include links from bibliography back to text
    maxbibnames=3, maxcitenames=2, % show all names in bibliography, but up to 2 in-text
    uniquelist=false, uniquename=false, % don't try to disambiguate name clashes in-text
    date=year, % don't include months in bibliography
    dashed=false, giveninits=true,
    sorting=nyt, sortcites=false, 
    isbn=false,doi=false,url=false,eprint=false, % don't include links (we will hyperlink the titles instead)
}{biblatex}
\RequirePackage{biblatex}

\DeclareNameAlias{sortname}{family-given} % Lastname, Firstname in reference list

% Simplify references by removing superfluous fields.
% remove publisher for everything other than books.
\AtEveryBibitem{
 \clearlist{address}
 \clearfield{date}
 \clearfield{eprint}
 \clearfield{isbn}
 \clearfield{issn}
 \clearlist{location}
 \clearfield{month}
 \clearfield{series}
 \clearname{editor}
 
 \ifentrytype{book}{}{
   \clearlist{publisher}
 }
}

% use '&' instead of 'and' for consistency with natbib
\renewcommand*{\finalnamedelim}{%
    \ifnumgreater{\value{liststop}}{2}{\finalandcomma}{}%
    \addspace\&\space}%

% backref format
\DefineBibliographyStrings{english}{backrefpage={cited on p.},backrefpages={cited on pp.}} 

\renewcommand*{\bibfont}{\normalfont\footnotesize} % make bibliography use \small text
\setlength\bibitemsep{0.1\baselineskip} % increase spacing between items in bibliography

% --- Make title a hyperlink to the DOI (falls back to URL)
\newbibmacro{string+doiurl}[1]{%
  \iffieldundef{doi}{%
    \iffieldundef{url}{%
      \PackageWarning{mybibliography}{Entry \thefield{entrykey} has no DOI or URL}%
      #1%
    }{%
      \href{\thefield{url}}{#1}%
    }%
  }{%
    \href{http://dx.doi.org/\thefield{doi}}{#1}%
  }%
}

\DeclareFieldFormat{title}{\usebibmacro{string+doiurl}{\mkbibemph{#1}}}
\DeclareFieldFormat[article,incollection,misc,inproceedings,book]{title}%
    {\usebibmacro{string+doiurl}{\mkbibquote{#1}}}
% ---

% --- Make biblatex hyperlinks cover the name and year instead of just year (for consistency with natbib)
\DeclareFieldFormat{citehyperref}{%
  \DeclareFieldAlias{bibhyperref}{noformat}% Avoid nested links
  \bibhyperref{#1}}

\DeclareFieldFormat{textcitehyperref}{%
  \DeclareFieldAlias{bibhyperref}{noformat}% Avoid nested links
  \bibhyperref{%
    #1%
    \ifbool{cbx:parens}
      {\bibcloseparen\global\boolfalse{cbx:parens}}
      {}}}

\savebibmacro{cite}
\savebibmacro{textcite}

\renewbibmacro*{cite}{%
  \printtext[citehyperref]{%
    \restorebibmacro{cite}%
    \usebibmacro{cite}}}

\renewbibmacro*{textcite}{%
  \ifboolexpr{
    ( not test {\iffieldundef{prenote}} and
      test {\ifnumequal{\value{citecount}}{1}} )
    or
    ( not test {\iffieldundef{postnote}} and
      test {\ifnumequal{\value{citecount}}{\value{citetotal}}} )
  }
    {\DeclareFieldAlias{textcitehyperref}{noformat}}
    {}%
  \printtext[textcitehyperref]{%
    \restorebibmacro{textcite}%
    \usebibmacro{textcite}}}
% ---
